Multi-Interest-Aware User Modeling for Large-Scale Sequential Recommendations

Precise user modeling is critical for online personalized recommendation services. Generally, users' interests are diverse and are not limited to a single aspect, which is particularly evident when their behaviors are observed for a longer time. For example, a user may demonstrate interests in cats/dogs, dancing and food \& delights when browsing short videos on Tik Tok; the same user may show interests in real estate and women's wear in her web browsing behaviors. Traditional models tend to encode a user's behaviors into a single embedding vector, which do not have enough capacity to effectively capture her diverse interests. This paper proposes a Sequential User Matrix (SUM) to accurately and efficiently capture users' diverse interests. SUM models user behavior with a multi-channel network, with each channel representing a different aspect of the user's interests. User states in different channels are updated by an \emph{erase-and-add} paradigm with interest- and instance-level attention. We further propose a local proximity debuff component and a highway connection component to make the model more robust and accurate. SUM can be maintained and updated incrementally, making it feasible to be deployed for large-scale online serving. We conduct extensive experiments on two datasets. Results demonstrate that SUM consistently outperforms state-of-the-art baselines.

==> reference-complete.tex <==

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

%Entries

@inproceedings{10.1145/3097983.3098108,
author = {Okura, Shumpei and Tagami, Yukihiro and Ono, Shingo and Tajima, Akira},
title = {Embedding-Based News Recommendation for Millions of Users},
year = {2017},
isbn = {9781450348874},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3097983.3098108},
doi = {10.1145/3097983.3098108},
booktitle = {Proceedings of the 23rd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {1933–1942},
numpages = {10},
keywords = {distributed representations, neural networks, large-scale services, news recommendations},
location = {Halifax, NS, Canada},
series = {KDD ’17}
}

@inproceedings{liu2019hi,
  title={Hi-Fi ark: deep user representation via high-fidelity archive network},
  author={Liu, Zheng and Xing, Yu and Wu, Fangzhao and An, Mingxiao and Xie, Xing},
  booktitle={Proceedings of the 28th International Joint Conference on Artificial Intelligence},
  pages={3059--3065},
  year={2019},
  organization={AAAI Press}
}

@inproceedings{ren2019lifelong,
  title={Lifelong Sequential Modeling with Personalized Memorization for User Response Prediction},
  author={Ren, Kan and Qin, Jiarui and Fang, Yuchen and Zhang, Weinan and Zheng, Lei and Bian, Weijie and Zhou, Guorui and Xu, Jian and Yu, Yong and Zhu, Xiaoqiang and others},
  booktitle={Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={565--574},
  year={2019}
}

@inproceedings{DBLP:journals/corr/WestonCB14,
  author    = {Jason Weston and
               Sumit Chopra and
               Antoine Bordes},
  title     = {Memory Networks},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  crossref  = {DBLP:conf/iclr/2015},
  url       = {http://arxiv.org/abs/1410.3916},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/WestonCB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/iclr/2015,
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  url       = {https://iclr.cc/archive/www/doku.php\%3Fid=iclr2015:accepted-main.html},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/2015.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{wang2019modeling,
  title={Modeling multi-purpose sessions for next-item recommendations via mixture-channel purpose routing networks},
  author={Wang, Shoujin and Hu, Liang and Wang, Yang and Sheng, Quan Z and Orgun, Mehmet and Cao, Longbing},
  booktitle={Proceedings of the 28th International Joint Conference on Artificial Intelligence},
  pages={1--7},
  year={2019},
  organization={AAAI Press}
}

@inproceedings{li2019multi,
  title={Multi-interest network with dynamic routing for recommendation at Tmall},
  author={Li, Chao and Liu, Zhiyuan and Wu, Mengmeng and Xu, Yuchi and Zhao, Huan and Huang, Pipei and Kang, Guoliang and Chen, Qiwei and Li, Wei and Lee, Dik Lun},
  booktitle={Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
  pages={2615--2623},
  year={2019}
}

@article{DBLP:journals/corr/GravesWD14,
  author    = {Alex Graves and
               Greg Wayne and
               Ivo Danihelka},
  title     = {Neural Turing Machines},
  journal   = {CoRR},
  volume    = {abs/1410.5401},
  year      = {2014},
  url       = {http://arxiv.org/abs/1410.5401},
  archivePrefix = {arXiv},
  eprint    = {1410.5401},
  timestamp = {Mon, 13 Aug 2018 16:46:28 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/GravesWD14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pi2019practice,
  title={Practice on long sequential user behavior modeling for click-through rate prediction},
  author={Pi, Qi and Bian, Weijie and Zhou, Guorui and Zhu, Xiaoqiang and Gai, Kun},
  booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2671--2679},
  year={2019}
}

@inproceedings{chen2018sequential,
  title={Sequential recommendation with user memory networks},
  author={Chen, Xu and Xu, Hongteng and Zhang, Yongfeng and Tang, Jiaxi and Cao, Yixin and Qin, Zheng and Zha, Hongyuan},
  booktitle={Proceedings of the eleventh ACM international conference on web search and data mining},
  pages={108--116},
  year={2018}
}

@inproceedings{shen2014latent,
  title={A latent semantic model with convolutional-pooling structure for information retrieval},
  author={Shen, Yelong and He, Xiaodong and Gao, Jianfeng and Deng, Li and Mesnil, Gr{\'e}goire},
  booktitle={Proceedings of the 23rd ACM international conference on conference on information and knowledge management},
  pages={101--110},
  year={2014}
}

@inproceedings{koren2008factorization,
  title={Factorization meets the neighborhood: a multifaceted collaborative filtering model},
  author={Koren, Yehuda},
  booktitle={Proceedings of the 14th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={426--434},
  year={2008},
  organization={ACM}
}

@article{hidasi2015session,
  title={Session-based recommendations with recurrent neural networks},
  author={Hidasi, Bal{\'a}zs and Karatzoglou, Alexandros and Baltrunas, Linas and Tikk, Domonkos},
  journal={arXiv preprint arXiv:1511.06939},
  year={2015}
}
@inproceedings{hidasi2018recurrent,
  title={Recurrent neural networks with top-k gains for session-based recommendations},
  author={Hidasi, Bal{\'a}zs and Karatzoglou, Alexandros},
  booktitle={Proceedings of the 27th ACM International Conference on Information and Knowledge Management},
  pages={843--852},
  year={2018}
}

@inproceedings{10.1145/3109859.3109896,
author = {Quadrana, Massimo and Karatzoglou, Alexandros and Hidasi, Bal\'{a}zs and Cremonesi, Paolo},
title = {Personalizing Session-Based Recommendations with Hierarchical Recurrent Neural Networks},
year = {2017},
isbn = {9781450346528},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3109859.3109896},
doi = {10.1145/3109859.3109896},
booktitle = {Proceedings of the Eleventh ACM Conference on Recommender Systems},
pages = {130–137},
numpages = {8},
keywords = {recurrent neural networks, session-based recommendation, session-aware recommendation, personalization},
location = {Como, Italy},
series = {RecSys ’17}
}

@inproceedings{yu2019adaptive,
  title={Adaptive user modeling with long and short-term preferences for personalized recommendation},
  author={Yu, Zeping and Lian, Jianxun and Mahmoody, Ahmad and Liu, Gongshen and Xie, Xing},
  booktitle={Proceedings of the 28th International Joint Conference on Artificial Intelligence},
  pages={4213--4219},
  year={2019},
  organization={AAAI Press}
}
@inproceedings{10.1145/3292500.3330984,
author = {Ma, Chen and Kang, Peng and Liu, Xue},
title = {Hierarchical Gating Networks for Sequential Recommendation},
year = {2019},
isbn = {9781450362016},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3292500.3330984},
doi = {10.1145/3292500.3330984},
booktitle = {Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
pages = {825–833},
numpages = {9},
keywords = {feature gating, instance gating, item-item product, sequential recommendation},
location = {Anchorage, AK, USA},
series = {KDD ’19}
}
@inproceedings{10.1145/3308558.3313408,
author = {Xu, Chengfeng and Zhao, Pengpeng and Liu, Yanchi and Xu, Jiajie and S.Sheng, Victor S.Sheng and Cui, Zhiming and Zhou, Xiaofang and Xiong, Hui},
title = {Recurrent Convolutional Neural Network for Sequential Recommendation},
year = {2019},
isbn = {9781450366748},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3308558.3313408},
doi = {10.1145/3308558.3313408},
booktitle = {The World Wide Web Conference},
pages = {3398–3404},
numpages = {7},
keywords = {Recurrent Neural Network, Convolutional Neural Network., Sequential Recommendation},
location = {San Francisco, CA, USA},
series = {WWW ’19}
}
  
@inproceedings{zhou2019deep,
  title={Deep Interest Evolution Network for Click-Through Rate Prediction},
  author={Zhou, Guorui and Mou, Na and Fan, Ying and Pi, Qi and Bian, Weijie and Zhou, Chang and Zhu, Xiaoqiang and Gai, Kun},
   booktitle={Thirty-Third AAAI Conference on Artificial Intelligence},
  year={2019}
}
  
@article{koren2009matrix,
  title={Matrix factorization techniques for recommender systems},
  author={Koren, Yehuda and Bell, Robert and Volinsky, Chris},
  journal={Computer},
  number={8},
  pages={30--37},
  year={2009},
  publisher={IEEE}
}
@inproceedings{10.1145/3366423.3380190,
author = {Guo, Xueliang and Shi, Chongyang and Liu, Chuanming},
title = {Intention Modeling from Ordered and Unordered Facets for Sequential Recommendation},
year = {2020},
isbn = {9781450370233},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3366423.3380190},
doi = {10.1145/3366423.3380190},
booktitle = {Proceedings of The Web Conference 2020},
pages = {1127–1137},
numpages = {11},
keywords = {user intention, purchased motivation, sequential recommendation, preference drift},
location = {Taipei, Taiwan},
series = {WWW ’20}
}
 @inproceedings{li2017neural,
  title={Neural attentive session-based recommendation},
  author={Li, Jing and Ren, Pengjie and Chen, Zhumin and Ren, Zhaochun and Lian, Tao and Ma, Jun},
  booktitle={Proceedings of the 2017 ACM on Conference on Information and Knowledge Management},
  pages={1419--1428},
  year={2017},
  organization={ACM}
}
@inproceedings{10.1145/3289600.3290975,
author = {Yuan, Fajie and Karatzoglou, Alexandros and Arapakis, Ioannis and Jose, Joemon M. and He, Xiangnan},
title = {A Simple Convolutional Generative Network for Next Item Recommendation},
year = {2019},
isbn = {9781450359405},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3289600.3290975},
doi = {10.1145/3289600.3290975},
booktitle = {Proceedings of the Twelfth ACM International Conference on Web Search and Data Mining},
pages = {582–590},
numpages = {9},
keywords = {dilated cnn, session-based recommendation, sequence learning, convolutional neural network, residual learning},
location = {Melbourne VIC, Australia},
series = {WSDM ’19}
}
  
@inproceedings{tang2018personalized,
  title={Personalized top-n sequential recommendation via convolutional sequence embedding},
  author={Tang, Jiaxi and Wang, Ke},
  booktitle={Proceedings of the Eleventh ACM International Conference on Web Search and Data Mining},
  pages={565--573},
  year={2018}
}
@article{DBLP:journals/corr/abs-1808-06414,
  author    = {Shuai Zhang and
               Yi Tay and
               Lina Yao and
               Aixin Sun},
  title     = {Next Item Recommendation with Self-Attention},
  journal   = {CoRR},
  volume    = {abs/1808.06414},
  year      = {2018},
  url       = {http://arxiv.org/abs/1808.06414},
  archivePrefix = {arXiv},
  eprint    = {1808.06414},
  timestamp = {Mon, 19 Nov 2018 13:08:35 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1808-06414},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icdm/KangM18,
  author    = {Wang{-}Cheng Kang and
               Julian J. McAuley},
  title     = {Self-Attentive Sequential Recommendation},
  booktitle = {{IEEE} International Conference on Data Mining, {ICDM} 2018, Singapore,
               November 17-20, 2018},
  pages     = {197--206},
  year      = {2018}, 
  url       = {https://doi.org/10.1109/ICDM.2018.00035},
  doi       = {10.1109/ICDM.2018.00035},
  timestamp = {Mon, 22 Jul 2019 19:11:02 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/icdm/KangM18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{10.1145/3357384.3357895,
author = {Sun, Fei and Liu, Jun and Wu, Jian and Pei, Changhua and Lin, Xiao and Ou, Wenwu and Jiang, Peng},
title = {BERT4Rec: Sequential Recommendation with Bidirectional Encoder Representations from Transformer},
year = {2019},
isbn = {9781450369763},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3357384.3357895},
doi = {10.1145/3357384.3357895},
booktitle = {Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
pages = {1441–1450},
numpages = {10},
keywords = {cloze, sequential recommendation, bidirectional sequential model},
location = {Beijing, China},
series = {CIKM ’19}
}
  
@inproceedings{10.1145/3357384.3357818,
author = {Lv, Fuyu and Jin, Taiwei and Yu, Changlong and Sun, Fei and Lin, Quan and Yang, Keping and Ng, Wilfred},
title = {SDM: Sequential Deep Matching Model for Online Large-Scale Recommender System},
year = {2019},
isbn = {9781450369763},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3357384.3357818},
doi = {10.1145/3357384.3357818},
booktitle = {Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
pages = {2635–2643},
numpages = {9},
keywords = {deep matching, sequential recommendation},
location = {Beijing, China},
series = {CIKM ’19}
}
  
@inproceedings{cho-etal-2014-properties,
    title = "On the Properties of Neural Machine Translation: Encoder{--}Decoder Approaches",
    author = {Cho, Kyunghyun  and
      van Merri{\"e}nboer, Bart  and
      Bahdanau, Dzmitry  and
      Bengio, Yoshua},
    booktitle = "Proceedings of {SSST}-8, Eighth Workshop on Syntax, Semantics and Structure in Statistical Translation",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W14-4012",
    doi = "10.3115/v1/W14-4012",
    pages = "103--111",
}



@inproceedings{DBLP:conf/ijcai/GuoTYLH17,
  author    = {Huifeng Guo and
               Ruiming Tang and
               Yunming Ye and
               Zhenguo Li and
               Xiuqiang He},
  title     = {DeepFM: {A} Factorization-Machine based Neural Network for {CTR} Prediction},
  booktitle = {Proceedings of the Twenty-Sixth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2017, Melbourne, Australia, August
               19-25, 2017},
  pages     = {1725--1731},
  year      = {2017},
  crossref  = {DBLP:conf/ijcai/2017},
  url       = {https://doi.org/10.24963/ijcai.2017/239},
  doi       = {10.24963/ijcai.2017/239},
  timestamp = {Tue, 20 Aug 2019 16:16:54 +0200},
  biburl    = {https://dblp.org/rec/conf/ijcai/GuoTYLH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/ijcai/2017,
  editor    = {Carles Sierra},
  title     = {Proceedings of the Twenty-Sixth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2017, Melbourne, Australia, August
               19-25, 2017},
  publisher = {ijcai.org},
  year      = {2017},
  url       = {http://www.ijcai.org/Proceedings/2017/},
  isbn      = {978-0-9992411-0-3},
  timestamp = {Tue, 20 Aug 2019 16:16:54 +0200},
  biburl    = {https://dblp.org/rec/conf/ijcai/2017.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{wu2017recurrent,
  title={Recurrent recommender networks},
  author={Wu, Chao-Yuan and Ahmed, Amr and Beutel, Alex and Smola, Alexander J and Jing, How},
  booktitle={Proceedings of the tenth ACM international conference on web search and data mining},
  pages={495--503},
  year={2017}
}
@inproceedings{10.5555/3172077.3172393,
author = {Zhu, Yu and Li, Hao and Liao, Yikang and Wang, Beidou and Guan, Ziyu and Liu, Haifeng and Cai, Deng},
title = {What to Do next: Modeling User Behaviors by Time-LSTM},
year = {2017},
isbn = {9780999241103},
publisher = {AAAI Press},
booktitle = {Proceedings of the 26th International Joint Conference on Artificial Intelligence},
pages = {3602–3608},
numpages = {7},
location = {Melbourne, Australia},
series = {IJCAI’17}
}
  
@inproceedings{10.1145/3336191.3371786,
author = {Li, Jiacheng and Wang, Yujie and McAuley, Julian},
title = {Time Interval Aware Self-Attention for Sequential Recommendation},
year = {2020},
isbn = {9781450368223},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3336191.3371786},
doi = {10.1145/3336191.3371786},
booktitle = {Proceedings of the 13th International Conference on Web Search and Data Mining},
pages = {322–330},
numpages = {9},
keywords = {time-aware model, recommender system, self-attenion, sequential prediction},
location = {Houston, TX, USA},
series = {WSDM ’20}
}
  
@inproceedings{10.1145/3219819.3220023,
author = {Lian, Jianxun and Zhou, Xiaohuan and Zhang, Fuzheng and Chen, Zhongxia and Xie, Xing and Sun, Guangzhong},
title = {XDeepFM: Combining Explicit and Implicit Feature Interactions for Recommender Systems},
year = {2018},
isbn = {9781450355520},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3219819.3220023},
doi = {10.1145/3219819.3220023},
booktitle = {Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
pages = {1754–1763},
numpages = {10},
keywords = {deep learning, neural network, feature interactions, factorization machines, recommender systems},
location = {London, United Kingdom},
series = {KDD ’18}
}
  
@inproceedings{10.1145/3209978.3210017,
author = {Huang, Jin and Zhao, Wayne Xin and Dou, Hongjian and Wen, Ji-Rong and Chang, Edward Y.},
title = {Improving Sequential Recommendation with Knowledge-Enhanced Memory Networks},
year = {2018},
isbn = {9781450356572},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3209978.3210017},
doi = {10.1145/3209978.3210017},
booktitle = {The 41st International ACM SIGIR Conference on Research \& Development in Information Retrieval},
pages = {505–514},
numpages = {10},
keywords = {knowledge base, sequential recommendation, memory network},
location = {Ann Arbor, MI, USA},
series = {SIGIR ’18}
}
  
@inproceedings{10.1145/3397271.3401088,
author = {Liu, Zheng and Lian, Jianxun and Yang, Junhan and Lian, Defu and Xie, Xing},
title = {Octopus: Comprehensive and Elastic User Representation for the Generation of Recommendation Candidates},
year = {2020},
isbn = {9781450380164},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3397271.3401088},
doi = {10.1145/3397271.3401088},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {289–298},
numpages = {10},
keywords = {user representation, recommendation system, candidate generation, user modeling},
location = {Virtual Event, China},
series = {SIGIR ’20}
}
  
@article{cen2020controllable,
  title={Controllable Multi-Interest Framework for Recommendation},
  author={Cen, Yukuo and Zhang, Jianwei and Zou, Xu and Zhou, Chang and Yang, Hongxia and Tang, Jie},
  journal={arXiv preprint arXiv:2005.09347},
  year={2020}
}

@inproceedings{liu2005investigation,
  title={An investigation of practical approximate nearest neighbor algorithms},
  author={Liu, Ting and Moore, Andrew W and Yang, Ke and Gray, Alexander G},
  booktitle={Advances in neural information processing systems},
  pages={825--832},
  year={2005}
}

@inproceedings{deepxml,
author = {Dahiya, Kunal and  Saini, Deepak and  Mittal, Anshul and  Shaw, Ankush and  Dave, Kushal and  Soni, Akshay and  Jain, Himanshu and  Agarwal, Sumeet and  Varma, Manik},
title = {DeepXML: A Deep Extreme Multi-Label Learning Framework Applied to Short Text Documents},
year = {2021}, 
publisher = {Association for Computing Machinery}, 
series = {WSDM '21}
}

